McMule -- QED Corrections for Low-Energy Experiments

We present McMule, a unified framework for the calculation of NLO and NNLO corrections to many processes in QED with massive fermions. This easily extendable program allows users to calculate an arbitrary observable for any of the processes implemented. These include various lepton decays as well as certain low-energy scattering experiments such as $e\mu\to e\mu$ and $\ell p\to\ell p$ that can be measured to high enough a precision to warrant QED corrections. As part of our discussion, we will present a pedagogical introduction to how these calculations are performed, focusing on technical aspects supplemented with examples. Our goal is to provide a useful introduction for those entering the field, covering all aspects relevant for the practitioner.

==> figures/tikz/muondecay-proto.tex <==
%!TEX root=thesis
%PDFLATEX

\newcommand{\drawd}[1]{
\begin{tikzpicture}
 
 \coordinate (muin) at (180:3.0);
 \coordinate (eout) at (-45:3.0);
 \coordinate (vert) at (  0,0.0);
 \coordinate (qed1) at (180:1.5);
 \coordinate (qed2) at (-45:1.5);
 \node    at (muin)[left ] {$\mu^-$};
 \node    at (eout)[right] {$e  ^-$};

 \draw[mfermion] (muin) -- (qed1) -- (vert) -- (qed2) -- (eout);
 \draw[mfermion,dashed] (30:2) -- (45:0.2) -- (60:2);
 
 \centerarc[#1](0,0)(135:0:-1.5)
 
 \draw[->,thick] (muin) ++ (45:0.4) --+ (  0:0.8) node [above,midway] {\scalebox{0.6}{$   p $}};
 \draw[->,thick] (qed1) ++ (45:0.4) --+ (  0:0.8) node [above,midway] {\scalebox{0.6}{$(p-k)$}};
 \draw[->,thick] (vert) ++ ( 0:0.4) --+ (-45:0.8) node [right,midway] {\scalebox{0.6}{$(q-k)$}};
 \draw[->,thick] (qed2) ++ ( 0:0.4) --+ (-45:0.8) node [right,midway] {\scalebox{0.6}{$   q $}};
 \centerarc[<-,thick](0,0)(80:55:-1.9); \node at (67.5:-2.2)          {\scalebox{0.6}{$ k   $}};
\end{tikzpicture}
}

